Synthesis from Formal Partial Abstractions

Developing complex software systems is costly, time-consuming and error-prone. Model- driven development (MDD) promises to improve software productivity, timeliness, quality and cost through the transformation of abstract application models to code-level implementations. However, it remains unreasonably difficult to build the modeling languages and translators required for software synthesis. This difficulty, in turns, limits the applicability of MDD, and makes it hard to achieve reliability in MDD tools. This dissertation research seeks to reduce the cost, broaden the applicability, and increase the quality of model-driven development systems by embedding modeling languages within established formal languages and by using the analyzers provided with such languages for synthesis purposes to reduce the need for hand coding of translators. This dissertation, in particular, explores the proposed approach using relational logic as expressed in Alloy as the general specification language, and the Alloy Analyzer as the general-purpose analyzer. Synthesis is thus driven by finite-domain constraint satisfaction. One important aspect of this work is its focus on partial specifications of particular aspects of the system, such as application architectures and target platforms, and synthesis of partial code bases from such specifications. Contributions of this work include novel insights, methods and tools for (1) synthesizing architectural models from abstract application models; (2) synthesizing partial, platform-specific application frameworks from application architectures; and (3) synthesizing object-relational mapping tradeoff spaces and database schemas for database-backed object-oriented applications.

==> chapter4.bak.tex <==
\chapter{Formal Synthesis of Tradeoff Spaces for Object-Relational Mapping}

Relational database and object-oriented software development are both playing central roles in their respective areas.  Object-oriented applications often need to use relational databases for persistent storage. Transformations between instance models in these two paradigms encounter the so-called {\em impedance mismatch} problem~\cite{ireland_understanding_2009}. Object-relational mapping (ORM) systems are now widely used to bridge the gap between object-oriented application models and relational database management systems (DBMS), based on application-specific mapping definitions on how object models are to be mapped to database structures.

The problem is that today one has to choose between automatic generation of mappings using \emph{pure} mapping patterns~\cite{luca_cabibbo_managing_2005,ireland_understanding_2009}, or the manual design of mixed mappings, in which different mapping strategies are applied to individual classes rather than to entire inheritance hierarchies. Producing pure mappings automatically is easy, but it often leads to sub-optimal results. Developing mixed mappings by hand can achieve much higher quality, but it is hard and error-prone. Among other things, it requires a thorough understanding of both object and relational paradigms, of large spaces of possible mappings, and of the tradeoffs involved in making choices in these spaces.

To address this problem, I present a novel approach that provides both the quality benefits of mixed mappings and the productivity benefits of automated synthesis. I present a practical formal automated technique, implemented in a prototype tool called {\em Spacemaker}, for exhaustive synthesis of mixed OR mappings and their classification into quality attribute equivalence classes.
It takes as inputs a formal object model and optional class-specific mapping strategies for those classes that the user wants mapped in a specific manner.
%We take a formal object model as input, including optional class-specific mapping strategies for classes that the user wants mapped in a specific manner.
It then uses an automated constraint solver to exhaustively generate the space of mappings subject to the given constraints, along with multiple quality attribute measures for each mapping. Next it clusters mappings into quality attribute equivalence classes and presents candidates from each class to the engineer along with the measures of its quality attributes. The engineer can then select a mapping to satisfy tradeoff preferences. The prototype tool uses Alloy as a specification language~\cite{daniel_jackson_alloy:lightweight_2002}, and the Alloy analyzer as a constraint solver.

%This paper makes four principal contributions.
In more detail, I claim four main contributions for this part of my research:
(1) I present what is to my knowledge the first formalization of fine-grained and mixed ORM strategies by means of mapping functions; (2) I contribute a fully automated approach for formally precise synthesis of mapping tradeoff spaces, based on this formalization; (3) I present an experimental demonstration of technical feasibility and scalability to practically meaningful applications; and (4) I develop the Spacemaker tool~\cite{_spacemaker}, which I make available to the research and education community.
Data collected from the experiments support the claim that this technique can reduce the time to develop high-quality OR mappings, ensure their correctness, and enable engineers to make tradeoffs based on automatically computed quality attributes for a full range of possible mappings rather than on intuition or hard-to-acquire expertise in OR mapping strategies.

The rest of this chapter is organized as follows.
Section~\ref{Approach} presents the approach.
Section~\ref{evaluation} reports and discusses data from the experimental testing of the approach.
Section~\ref{related} surveys related efforts.
Section~\ref{conclusion} concludes with an outline of future work in line this research component.
%Finally, the paper concludes with an outline of our future work.
%Section~\ref{conclusion} concludes and discusses future work.


\section{Approach}
\label{Approach}

I present the approach in four parts.
I first introduce \emph{Alloy-OM}, a domain-specific language that I developed within the Alloy language to let developers specify object models in Alloy. Next, I present formalizations of object-relational mapping strategies, and then use these formalizations to automate synthesis of quality equivalence classes of OR mappings.
%We finally detail our algorithm for decomposing object models to improve scalability.
Finally, I describe algorithms that are important for the scalability of the approach.
In a nutshell, they serve to decompose large object models into smaller components for which mapping problems can be solved independently. This element of the work helps avoid combinatorial explosion in constraint solving.



\subsection{Alloy-OM}
The Alloy object model (Alloy-OM) is a domain specific language (DSL), I developed in Alloy. The user of Spacemaker then can describe object models in the Alloy-OM DSL. The Alloy-OM meta-model has three main constructs: Class, Attribute and Association. For each class in the object model, there is a corresponding ``Class'' signature in the Alloy-OM model. Similarly, for each attribute of a given class in the object model, the corresponding Alloy-OM Class signature contains a corresponding Alloy-OM Attribute as a member of its attribute set. Finally, each association in the object model has a corresponding ``Association'' signature in the Alloy-OM model. In the following, I will describe details of each of these elements.

\subsubsection{Class Definition}

Each Class signature in the Alloy-OM model has a set of fields: attrSet, id, parent and isAbstract. The ``attrSet'' field in each Class signature specifies the set of attributes as defined for the corresponding class in the object model. The ``id'' field in the Class signature represents the identifier of the corresponding class. The inheritance relationship in the object model is represented by the ``parent'' relation in the Alloy-OM model. Specifically, the inheritance relationship between classes c and p, where c inherits from p, will represent by the expression of ``\emph{parent = p}'' specified within the c class signature definition. Finally, ``isAbstract'' field of each Alloy-OM class signature denotes whether the class under consideration is abstract or not.


\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-25pt}
  \begin{center}
    \includegraphics[width=0.53\textwidth]{Pics/ch4/customer-orderObjectModel.png}
  \end{center}
%  \vspace{-25pt}
  \caption{\label{fig:object_model_diagram}customer-order object model.
  }
%\vspace{-0.6cm}
%\vspace{-15pt}
\end{wrapfigure}


To make the idea concrete, Figure~\ref{fig:object_model_diagram} shows an object model diagram for a simple customer-order example. The object model contains three classes of Order, Customer, and PreferredCustomer. There is a one-to-many association between the Customer and Order classes, and PreferredCustomer inherits from the Customer class.



To describe each class in the Alloy-OM, I define a signature that extends ``Class'' signature defined within the Alloy-OM meta-model. For example, Listing~\ref{orderClass} represents ``Order'' class in Alloy-OM DSL.

\begin{figure}
\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=left,                   % where to put the line-numbers
numberstyle=\tiny,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=7pt,%5pt,            % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=bottomline, %none, %single            % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
xleftmargin=1.5em,
%title=\lstname,                 % show the filename of files included with \lstinputlisting; also try caption instead of title
%escapeinside={\%*}{*)}          % if you want to add a comment within your code
%morekeywords={*,...}            % if you want to add more keywords to the set
morekeywords={module,sig,abstract,extends,one,some,set,open,pred,all,in,no}
}
\lstinputlisting[caption=Order class in Alloy-OM.,numberbychapter=false,label=orderClass]
%{Arch_model_Alloy.als}
{Pics/ch4/Order-class.als}
\vspace{-0.6cm}
\end{figure}


The order class has two attributes of ``orderID'' and ``orderValue'', which are assigned to the ``attrSet'' field of the Order class. The id field specifies the orderID as the identifier of this class. The last two lines of the Order signature specification denote that Order is not an abstract class and has no parent.
Similarly, the following code snippet represents ``PreferredCustomer'' signature definition. According to Fig.~\ref{fig:object_model_diagram}, this class inherits from the Customer class. The expression on line 3, thus, specifies Customer as the parent of the PreferredCustomer class.

\begin{figure}
\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=left,                   % where to put the line-numbers
numberstyle=\tiny,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=7pt,%5pt,            % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=bottomline, %none, %single            % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
xleftmargin=1.5em,
%title=\lstname,                 % show the filename of files included with \lstinputlisting; also try caption instead of title
%escapeinside={\%*}{*)}          % if you want to add a comment within your code
%morekeywords={*,...}            % if you want to add more keywords to the set
morekeywords={module,sig,abstract,extends,one,some,set,open,pred,all,in,no}
}
\lstinputlisting[caption=PreferredCustomer class in Alloy-OM.,numberbychapter=false,label=PreferredCustomer]
%{Arch_model_Alloy.als}
{Pics/ch4/PreferredCustomer.als}
\vspace{-0.6cm}
\end{figure}


\subsubsection{Attribute Definition}

To describe each attribute in the Alloy-OM, I define a signature that extends the corresponding data type signature. Alloy-OM DSL contains a set of predefined data types, namely Integer, Real, string and Bool. As a concrete example, orderValue is an attribute of type Real for the Order Class. The following code snippet represents its specification in Alloy-OM:
\emph{one sig orderValue extends Real{}}

The user can also specify a new data type by defining an abstract signature that extends the ''Type'' signature. The following expression defines a data type named NewDataType.
\emph{abstract sig NewDataType extends Type{}}



\subsubsection{Association Definition}

Each Association signature in the Alloy-OM model has four fields: src, dst, $src\_multiplicity$ and $dst\_multiplicity$. The src and dst fields of each Association signature specify the source and destination classes for that association, respectively. Association multiplicity defines the number of object instances that can be at each end of the association. The $src\_multiplicity$ and $dst\_multiplicity$ fields represent Association multiplicities of source and destination classes respectively, and can have values of either ONE or MANY.


\begin{figure}[bh]
\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=left,                   % where to put the line-numbers
numberstyle=\tiny,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=7pt,%5pt,            % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=bottomline, %none, %single            % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
xleftmargin=1.5em,
%title=\lstname,                 % show the filename of files included with \lstinputlisting; also try caption instead of title
%escapeinside={\%*}{*)}          % if you want to add a comment within your code
%morekeywords={*,...}            % if you want to add more keywords to the set
morekeywords={module,sig,abstract,extends,one,some,set,open,pred,all,in,no}
}
\lstinputlisting[caption=CustomerOrder Association in Alloy-OM.,numberbychapter=false,label=CustomerOrderAssociation]
%{Arch_model_Alloy.als}
{Pics/ch4/CustomerOrderAssociation.als}
\vspace{-0.6cm}
\end{figure}

As a concrete example, to describe the association between customer and order in the Alloy-OM model, I define a corresponding signature that extends ``Association'' signature. The code snippet of Listing~\ref{CustomerOrderAssociation} represents CustomerOrderAssociation specification in the Alloy-OM.
The above specification states Customer and Order classes as source and destination of the CustomerOrder association, respectively. The CustomerOrderAssociation is a ``one-to-many'' association, which is specified using $src\_multiplicity$ and $dst\_multiplicity$ fields.

Now, we have all the elements to specify the customer-order object model diagram in the Alloy-OM DSL. Putting all together, the specification of the Alloy-OM model for the customer-order example is represented in Fig.~\ref{fig:customerOrderAlloyOM}. The alloy module starts by specifying the name of the model, here module customerOrderObjectModel. We then import the Alloy-OM declaration module by the following expression: open Declaration. The rest of the module specifies three classes, their attributes and the association between Customer and Order classes.

\begin{figure}[tbh]
\centering
%\includegraphics[width=3.5in]{impl_model_Pics/impl_model_2_2_Labeled_3_5_change_color_text_2-resized}
%\includegraphics[width=3.5in]{Pics/ch3/impl_model_2_2.png}
\includegraphics[width=6in]{Pics/ch4/customerOrderAlloyOM.png}
\caption{\label{fig:customerOrderAlloyOM}
customer-order Alloy-OM model.
}
\end{figure}


\begin{comment}
Finally, to find instances of our Alloy-OM model, we can add a predicate and a command, as follows:
pred show{}
run show for 2 but 8 Attribute
The show predicate has an empty body, as we do not need to add any more constraint to our model. The run command specifies a scope that bounds the search for instances. In this case, to at most two objects in each signature except for Attribute limited to eight objects, as we consider each class as an Attribute Type. It is worth mentioning that the scope is for the purpose of simulation alone, and the object-relational mapping does not depend on it.
\end{comment}



\subsection{Formalization}

The issue of mapping an object model to a set of relations is described thoroughly in the research literature~\cite{luca_cabibbo_managing_2005,ireland_understanding_2009,keller_mapping_1997,philippi_model_2005}.
To provide a basis for precise modeling of the space of mapping alternatives, I have formalized OR mapping strategies in an appropriate level of granularity.
As an enabling technology, I chose Alloy~\cite{daniel_jackson_alloy:lightweight_2002} as a specification language and satisfaction engine for three reasons.
First, its logical and relational operators makes Alloy an appropriate language for specifying object-relational mapping strategies. Second, its ability to compute solutions that satisfy complex constraints is useful as an automation mechanism. Third, Alloy has a rigorously defined semantics closely related to those of relational databases, thereby providing a sound formal basis for our approach.

The principal mapping strategies are explained in terms of the notations suggested by Philippi~\cite{philippi_model_2005}, and Cabibbo and Carosi~\cite{luca_cabibbo_managing_2005}.
To manage association relationships, I have formally specified three ORM strategies of {\em own association table}, {\em foreign key embedding} and {\em merging into single table}. I have also defined three more ORM strategies for inheritance relationships: {\em class relation inheritance (CR)}, {\em concrete class relation inheritance (CCR)} and {\em single relation inheritance (SR)}. Furthermore, as the aforementioned ORM strategies for inheritance relationships are just applicable to the whole inheritance hierarchies, I have defined extra predicates for more fine-grained strategies: {\em Union Superclass}, {\em Joined Subclass} and {\em Union Subclass}, suitable to be applied to part of inheritance hierarchies, letting the developer design a detailed mapping specification using the combination of various ORM strategies.
To make the idea concrete, I illustrate the semantics of one of these strategies in the following.

\begin{figure}
\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=left,                   % where to put the line-numbers
numberstyle=\scriptsize ,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=bottomline,                    % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
xleftmargin=1.8em,
morekeywords={module,sig,abstract,extends,one,set,open,pred,all,in,none}
}
\lstinputlisting[caption=Part of the Alloy predicate for the $UnionSubclass$ strategy,numberbychapter=false,label=CCR]
{Pics/ch4/UnionSubclass_2.txt}
\vspace{-0.6cm}
\end{figure}

Listing~\ref{CCR} partially outlines the Alloy predicate for the {\em Union Subclass} strategy, where each concrete class within the hierarchy is represented by a separate table. The strategy predicate then states, in lines 5--14, %4--11,
that each table encompasses relational fields corresponding to both attributes of the associated class and its inherited attributes. As such, to retrieve an individual object, only one table needs to be accessed.
Finally, this strategy implies no referential %foreign key
constraint over the mapped relations.


\subsection{Design Space Exploration}
\label{DSE}
%In previous section, we showed how executable specifications can be used to formalize and automate application of ORM strategies.
In the previous section, I showed how analyzable specifications can be used to formalize OR mapping strategies.
In this section, I tackle the other aspect that needs to be clarified:
how one can apply a design space exploration approach to generate \emph{quality equivalence classes} of OR mappings based on those specifications.

A design space is a set of possible design alternatives, and design space exploration (DSE) is the process of traversing the design space to determine particular design alternatives that not only satisfy various design constraints, but are also optimized in the presence of a set of objectives~\cite{saxena_mde-based_2010}.
The process can be broken down into three key steps:
(1) Modeling the space of mapping alternatives;
(2) Evaluating each alternative by means of a set of metrics;
(3) Traversing the space of alternatives to cluster it into equivalence classes.


\subsection*{Modeling the Space of Mapping Alternatives}
For each application object model, due to a large number of mapping options available for each class, its attributes and associations, and its position in the inheritance hierarchy, there are several valid variants.
To model the space of all mapping alternatives, I develop a generic mixed mapping specification based on fine-grained strategies formalized in previous section.
This generic mixed mapping specification lets the automatic model finder choose for each element of the object model any of the relevant strategies, e.g. any of the fine-grained generalization mapping strategies for a given class within an inheritance hierarchy.

Applying such a loosely constrained mixed mapping strategy into the object model leads to a set of ORM specifications constituting the design space.
% Hazf
While they all represent the same object model and are consistent with the rules implied by a given mixed mapping strategy, they exhibit totally different quality attributes. For example, how inheritance hierarchies are being mapped to relational models affects the required space for data storage and the required time for query execution.

I called this mapping strategy loosely constrained because it does not concretely specify the details of the mapping, such as applying, for example the \emph{UnionSubclass} strategy to a specific class.
An expert user, though, is able to define a more tightly constrained mixed mapping by means of the parameterized predicates \emph{Spacemaker} provides, as I demonstrate in the next section.
The more detailed the mapping specifications, the narrower the outcome design space, and the less the required postprocessing search.


\subsection*{Measuring Impacts of OR mappings}

Mapping strategies have various kinds of impacts in terms of quality attributes of applications.
There are several approaches proposed in the literature dealing with the challenge of defining metrics for OR mapping impacts on non-functional characteristics.
It has been shown that efficiency, maintainability, and usability, among the set of all quality attributes defined by the ISO/IEC 9126-1 standard, are characteristics significantly influenced by OR mappings~\cite{stefan_holder_towardsmetrics_2008}.
For each of those attributes, I use a set of metrics suggested by Holder et al.~\cite{stefan_holder_towardsmetrics_2008} and Baroni et al.~\cite{baroni_formal_2005}. The metrics are \emph{Table Access for Type Identification} (\emph{TATI}), \emph{Number of Corresponding Table} (\emph{NCT}), \emph{Number of Corresponding Relational Fields} (\emph{NCRF}), \emph{Additional Null Value} (\emph{ANV}), \emph{Number of Involved Classes} (\emph{NIC}) and \emph{Referential Integrity Metric} (\emph{RIM}).


To measure these metrics, I developed a set of queries to execute over synthesized alternatives.
For brevity, and because it suffices to make the point, I concisely describe one of these metrics and the corresponding query in the following. \emph{Spacemaker} supports the others as well.


The \emph{Number of Corresponding Relational Fields} (NCRF) metric specifies the extent of change propagation for a given OR mapping. Specifically, the NCRF metric manifests the effort required to adapt a relational schema after applying a change, such as inserting or deleting an attribute, over a class. According to the definition, given a class \emph{C}, \emph{NCRF(C)} specifies the number of relational fields in all tables that correspond to each non-inherited, non-key attribute of \emph{C}.
The specification of a query we designated to measure the NCRF metric over synthesized alternatives is given below:

%\emph{NCRF(C) = \#(C.attrSet - C.id).~fAssociate.~fields}
\emph{NCRF(C) = \#(C.attrSet - C.id).$\sim$fAssociate.$\sim$fields}



The Alloy dot operator denotes a relational join.
While \emph{attrSet} specifies a set of non-inherited attributes of a class, \emph{fAssociate} is a relation from a table field to its associated class attribute. The query expressions then, by using the Alloy set cardinality operator \emph{(\#)}, defines the NCRF metric.



\subsection*{Exploring, Evaluating and Choosing}

The next step is to explore and prune the space of mapping alternatives according to quality measures.
Spacemaker partitions the space of satisfactory mixed mapping specifications into equivalence classes and selects at most a single candidate from each equivalence class for presenting to the end-user.

To partition the space, Spacemaker evaluates each alternative with respect to previously described relevant metrics. So each equivalence class consists of all alternatives that exhibit the same characteristics.
Specifically, two alternatives $a_1$ and $a_2$ are equivalent if \emph{value($a_1$, $m_i$)} = \emph{value($a_2$, $m_i$)} for all metrics ($m_i$). Because equivalent alternatives all satisfy the mapping constraints, it suffices to select one alternative in each equivalence class to find a choice alternative.
% Hazf
Given that quality characteristics are usually conflicting, there is generally no single optimum solution but there are several pareto-optimal choices representing best trade-offs.

\begin{comment}
\subsubsection*{Class Relation inheritance}
Using {\em class relation inheritance (CR)} strategy, each hierarchy is represented by a table for each class within the hierarchy.
Listing~\ref{CR} presents part of the predicate that represents {\em CR} strategy. According to lines 2--4, each table encompasses only relational fields corresponding to non-inherited attributes of the related class. That is, an object in the hierarchy is scattered over multiple tuples of different tables.
As mentioned in lines 7--10, tables associated to classes within a hierarchy share the same primary key, also considered as a foreign key from associated table of each subclass to its direct superclass corresponding table.

\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=left,                   % where to put the line-numbers
numberstyle=\scriptsize ,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,                    % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
xleftmargin=1.8em,
morekeywords={module,sig,abstract,extends,one,no,set,open,pred,all,in,none}
}


\lstinputlisting[caption=Part of the Alloy predicate for $CR$ strategy,numberbychapter=false,label=CR]
{ClassRelationInheritance.txt}

\end{comment}

\subsection{Transformation to Architecture Description Language}
\label{AlloyToSQLTransformer}


Having computed satisfying solutions, the \emph{Alloy2SQL transformer} component parses and transforms these solutions from low-level, XML formatted Alloy objects to high-level architecture descriptions in human-readable ADLs.
During the past several years, a considerable number of general and domain-specific ADLs have been proposed~\cite{nenad_medvidovic_classification_2000}. I use the Acme language in the prototype~\cite{david_garlan_acme:_2000}. Acme emerged as a generic language for describing software architectures, with particular support for architectural styles. It is also designed to work as an interchange format for mapping among other architecture description languages.


\subsection{Model Splitting}
As with many formal techniques, the complexity of constraint satisfaction restricts the size of models that can actually
be analyzed~\cite{ethan_k._jackson_components_2010}. This approach also requires an explicit representation of the set of all quality equivalence classes of mapping alternatives, which in general grows exponentially in the number of elements in a model.

To address these scalability problems, I split the object model into sub-models.
The key idea is that since for association relationships with cardinality of many-to-many, there is just one applicable mapping strategy, i.e. \emph{own association table}, I make use of such relations to split the object model into sub-models.




I consider an object model as a graph, $G_{objModel}= <V,E>$, where nodes \emph{V} represent classes,
and there is an edge $<v_i, v_j>$ joining two nodes $v_i$ and $v_j$ if there is a direct relationship including association and generalization link between them.
I assume that $G_{objModel}$ is connected. Otherwise, I consider each sub-graph separately.
An edge joining two nodes $v_i$ and $v_j$ in a graph is a \emph{bridge} if removing the edge would cause $v_i$ and $v_j$ to lie in two separate sub-graphs~\cite{david_easley_networks_2010}.
A bridge is the only route between its endpoints.
In other words, bridges provide nodes with access to parts of the graph that are inaccessible by other means.
So, to decompose a graph $G_{objModel}$, I remove all bridges of type many-to-many association.


\begin{figure*}[tbh]
\centering
\includegraphics[width=\linewidth]{Pics/ch4/newModel-2.png}
\caption{\label{fig:ecommerce}The ecommerce object model.}
\end{figure*}

To make the idea concrete I consider the ecommerce domain model adopted from Lau and Czarnecki~\cite{sean_quan_lau_domain_2006}.
According to the diagram shown in Figure~\ref{fig:ecommerce}, there are two such bridges: $<Product,Asset>$ and $<Item,Product>$.
By removing those bridges we obtain three smaller sub-graphs.
The gain then comes from the reduction in the sizes of the constraint solving problems. That is, I replace a large constraint solving problem with smaller and more manageable problems that can in particular be addressed by the formally precise synthesis technique.

\section{Evaluation}
\label{evaluation}

The claim I make for this work is twofold:
(1) It is feasible to formalize the \emph{correctness constraints} for object-relational mapping strategies, thereby to automate the synthesis of an exhaustive set of mixed object-relational mapping candidates, and that it is possible to statistically analyze each of the candidates in dimensions of six major mapping quality metrics, and thereby to cluster them into quality equivalence classes;
(2) for non-trivial systems, the performance of the technology implementation based on a bounded model checker is reasonable (on the order of minutes).

To test the feasibility hypothesis, I develop a prototype tool that implements it, called Spacemaker~\cite{_spacemaker}, which is available for download.
I show that the ideas are practical by applying Spacemaker to several case studies from the object-relational mapping literature.
I then compare the discrepancies between our formally derived OR mappings and the manual mappings published in the literature.
The differences revealed problems with their mappings, suggesting again that manual development of OR mappings can be error-prone.



\begin{figure*}[tbh]
\centering
\includegraphics[width=\linewidth]{Pics/ch4/Drawing4.png}
\caption{\label{fig:examples}Examples of mixed mapping strategies}
\end{figure*}

Figure~\ref{fig:examples} shows two applications of mixed ORM strategies, adopted from Holder et al.~\cite{stefan_holder_towardsmetrics_2008}.
White boxes represent classes, while boxes having grey titles represent corresponding mapped tables. Black and white arrows represent mapping and inheritance relationships, respectively. Finally, foreign keys as well as the applied mapping strategies are also mentioned in the diagrams.


Listing~\ref{appModel} formally describes part of the {\em personObjectModel} according to the diagram. At the top, it imports the declaration of {\em objectModel}, and then defines {\em Person} and its attribute, {\em name}, using signature extension as a subtype of {\em Class} and {\em Attribute} types. The other characteristics of the class are also specified.

\begin{figure}
\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=left,                   % where to put the line-numbers
numberstyle=\scriptsize ,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it's 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=bottomline,                    % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
%title=\lstname,                 % show the filename of files included with \lstinputlisting; also try caption instead of title
%escapeinside={\%*}{*)}          % if you want to add a comment within your code
%morekeywords={*,...}            % if you want to add more keywords to the set
morekeywords={module,sig,abstract,extends,one,no,set,open,pred,all,in,none}
}
\lstinputlisting[caption=Example of object model (elided) in Alloy,numberbychapter=false,label=appModel]
{Pics/ch4/appModel.txt}
\vspace{-0.6cm}
\end{figure}


\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=none,                   % where to put the line-numbers
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=none,                    % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=none,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
}
%\lstinputlisting[caption=High-level definition of mapping specifications]{singleRelationInheritance.txt}

To specify a mixed OR mapping, the developer can call fine-grained ORM strategies, given as inputs those classes to be mapped in a specific manner.
{\em Spacemaker} then automatically generates the corresponding mapping specifications, should they exist.
The followings outline the high-level definition of mapping specifications for Figure~\ref{fig:examples}a.

\begin{figure}[tbh]
\lstset{ %
basicstyle=\scriptsize,       % the size of the fonts that are used for the code \footnotesize\ttfamily
numbers=none,                   % where to put the line-numbers
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=none,                    % adds a frame around the code
tabsize=2,                    % sets default tabsize to 2 spaces
captionpos=none,                   % sets the caption-position to bottom
%captionpos=b,                   % sets the caption-position to bottom
breaklines=true,                % sets automatic line breaking
breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
numberbychapter=false,
%xleftmargin=0.2em%1.8em,
}
\lstinputlisting[caption=High-level definition of mapping specifications for figures~\ref{fig:examples}a and~\ref{fig:examples}b using our approach,numberbychapter=false,label=AlloyCode]
{Pics/ch4/mappingSpec.txt}
\vspace{-0.6cm}
\end{figure}


Figure~\ref{fig:AlloyModel} illustrates the computed result for the example of Figure~\ref{fig:examples}a.
The diagram is accurate for the result automatically computed, but I have edited it to omit some details for readability (fields of tables and primary key relationships, for example). In this diagram, Table 1 is associated to {\em Person} and {\em Employee} classes, which are being mapped by the {\em union superclass} strategy. Separate tables are associated to both {\em Student} and {\em Manager} classes, according to the {\em union subclass} strategy. Finally, application of the {\em joined subclass} strategy leads to a separate table for {\em Clerk} with a foreign key, omitted in the diagram, to its superclass corresponding table.


\begin{figure}[tbh]
\centering
\includegraphics[height=3.4in]{Pics/ch4/example2a-3.png}
%\includegraphics[height=3.0in]{Pics/example2a-3}
\caption{\label{fig:AlloyModel}Mapping diagram for Figure~\ref{fig:examples}a derived automatically based on mixed mapping strategies of {\em union superclass}, {\em joined subclass} and  {\em union subclass}}
\end{figure}
%[width=\linewidth] [width=\textwidth] [width=3.5in]


\begin{comment}
\begin{figure*}[tbh]
\centering
\includegraphics[width=\linewidth]{Pics/ch4/Outputs.png}
\caption{\label{fig:examples}Examples of mixed mapping strategies}
\end{figure*}
\end{comment}


To enumerate the space of mappings for the given object model, I use the \emph{genericMixedStrategy}, with the set of classes within the hierarchy as inputs. This generic strategy lets the automatic model finder, here Alloy analyzer, choose for each class any of the fine-grained strategies and to see whether their combinations applied to classes within the hierarchy is satisfiable or not.
Alloy guarantees that all computed mapping candidates conform to the rules implied by mapping predicates formalizing correctness constraints.

I used a PC with an Intel Core i5 2.67 Ghz processor and 4 GB of main memory, and leveraged \emph{SAT4J} as the SAT solver during the experiments.
Given all the specifications and mapping constraints, Spacemaker using the Alloy analyzer then generate 760,000 mapping candidates, assess them, and reduce them to 40 equivalence classes, in less than 10 seconds.




The spider diagram, shown in Figure~\ref{fig:spider_diagram}, illustrates the 6-dimensional ``quality measures'' for two mapping candidates represented in Figure~\ref{fig:examples}. To display quality measures in one diagram, I normalized the values.

\begin{comment}
\begin{figure}[tbh]
\centering
\includegraphics[width=3.4in]{Pics/ch4/Spider-diagram-2_2.png}
\caption{\label{fig:spider_diagram}Multi-dimensional \emph{quality measures} for two mapping candidates}
\end{figure}
\end{comment}

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-25pt}
  \begin{center}
    \includegraphics[width=0.53\textwidth]{Pics/ch4/Spider-diagram-2_2.png}
  \end{center}
%  \vspace{-25pt}
  \caption{\label{fig:spider_diagram}Multi-dimensional \emph{quality measures} for two mapping candidates %represented in Fig.~\ref{fig:examples}
  }
%\vspace{-0.6cm}
%\vspace{-15pt}
\end{wrapfigure}


According to the diagram, if the designer opts for the resource utilization, the mapping depicted in Figure~\ref{fig:examples}a would be a better option. More specifically, with respect to the ANV metric, representing additional storage space in terms of null values, the mapping of Figure~\ref{fig:spider_diagram}b requires more \emph{wasted space}. This is because instances of four different classes, namely Person, Student, Employee and Clerk, are stored together in a shared table. Thus, each row in the shared table that represents an instance of the Student class, for example, contains a null value at each relational field corresponding to the other classes. On the other hand, if the designer opts for maintainability and performance, the mapping depicted in Figure~\ref{fig:examples}b would be a better choice.
More precisely, the mapping of Figure~\ref{fig:examples}a negatively affects the NCRF metric reflecting the effort required to adapt the relational schema. This is partly because applying the \emph{UnionSubclass} strategy results in duplication of relational fields. With respect to the TATI metric which is a performance indicator of polymorphic database queries, this mapping also poses performance problems.


Focusing on the second hypothesis, to test that Spacemaker is able to handle also non-trivial OR mappings, I select an object model of a real ecommerce system~\cite{sean_quan_lau_domain_2006}. This object model, shown in Figure~\ref{fig:ecommerce}, represents a common architecture for the kind of open source and commercial ecommerce systems. It includes 15 classes connected by 9 associations and consists of 7 inheritance relationships.


Without decomposition, the Alloy analyzer ran out of memory before synthesizing the whole space of mapping alternatives. Given the splitting algorithm, we decompose the object model to three sub-models and feed them into the Spacemaker. Figure~\ref{fig:e_example} represents the results.

\begin{figure}[bth]
\centering
\begin{tabular}{|c||c|c|c|c|c|}
  \hline
  ObjectModel & Solutions &Eq.Classes& {$T [min]$} \\
  \hline
  Product & 137,000 & 67 & 46 \\
  \hline
  Asset & 124,000 & 31 & $1>$ \\
  \hline
  Order & 93,000 & 31 & 16 \\ %\cline{1-1} \cline{3-5} % Fig_a
  \hline
\end{tabular}
\caption{\label{fig:e_example}Ecommerce Experiment performance statistics.}
\end{figure}


Interpretation of data shows that similar to the former experiment, the synthesis time for the \emph{Asset} sub-model is in the order of seconds, but for the other two sub-models is in the order of minutes.
This is mainly because in the former case, the analyzer just considers inheritance mapping strategies as there are no associations in those models, while in the other models the constraints of both inheritance and association mapping strategies are involved. So it takes more time for the model finder to generate satisfying solutions for them.

As Spacemaker solves sub-models separately, the constraint solving bottleneck depends on the largest sub-model to solve.
Although the number of valid solutions is high, i.e. hundreds of thousands of satisfiable solutions, Spacemaker is able to generate quality equivalence classes of mappings in an acceptable amount of time, which confirms that the proposed synthesis technology is feasible.

\subsection*{Discussion}
\label{discussion}


This work shows that ORM strategies can be formalized and implemented as executable specifications, and that Spacemaker can automatically synthesize and prune the space of mapping alternatives in an effective manner.
The formal recapitulations of previous studies also reveals some problems. For example, the referential integrity constraint in Figure~\ref{fig:examples}b, is not mentioned in the source paper~\cite{stefan_holder_towardsmetrics_2008}, but exists in the mapping specifications automatically derived using {\em Spacemaker}.
Discovery of such inconsistencies provides an example of how formal synthesis technique can help designers in an error-prone task of developing OR mappings.

%Our goal is, however, not to develop another OR mapping middleware platform. Instead, we propose a novel approach aiming at the shortcomings of such platforms, by automatic generation of application-specific OR mapping specifications that regulate those platforms.



Overall, this work appears to support the idea that shifting the responsibility of finding an optimized mapping specification from technicians---who better understand mapping strategies, their implications, and techniques for mapping object models to relational models---to the domain experts, more aware of requirements and specifications
is a plausible aspiration.



\begin{comment}
\section{Related Work}
\label{related}
I can identify in the literature two categories of work that are closely related to this research.
The first one concerns the research that deals with deriving database-centric implementations from Alloy specification. The second one encompasses all works that have been done in the object-relational mapping research area.

Focusing on the first category, Krishnamurthi et al.~\cite{krishnamurthi_alchemy:_2008_short} proposed an approach to refine Alloy specifications into PLT Scheme implementations with special focus on persistent databases. Cunha and Pacheco~\cite{cunha_mapping_2009} are similarly focused on translating a subset of Alloy into the corresponding relational database operations. These works share with ours an emphasis on using formal methods. However, our work differs in its focus on separating application description from other independent design decisions, such as choices of OR mapping strategies. Furthermore, I use Alloy not only to specify the object model, but also to model the spaces of OR mappings consistent with both the given object model and choice mapping strategy, and to automate the mapping process.

Regarding the second area, a large body of work has focused on  object-relational mapping strategies and their impacts to address the impedance mismatch
problem~\cite{luca_cabibbo_managing_2005,ireland_understanding_2009,keller_mapping_1997,philippi_model_2005}. Among others,
Philippi~\cite{philippi_model_2005} categorized the mapping strategies in a set of pre-defined quality trade-off levels, which are used to develop a model driven approach for the generation of OR mappings. Cabibbo and Carosi~\cite{luca_cabibbo_managing_2005} also discussed more complex mapping strategies for inheritance hierarchies, in which the various strategies can be applied independently to different parts of a multi-level hierarchy.
I share the same problem domain with these approaches, but our focus is on automating formal derivation of equivalence classes of mapping specifications.



Drago et al.~\cite{drago_quality_2011} also considered OR mapping strategy as one of the variation points in their work on feedback provisioning. They extended the QVT-relations language with annotations for describing design variation points, and provided a feedback-driven backtracking capability to enable engineers to explore the design space.
While this work is concerned with the performance implications of choices of per-inheritance-hierarchy OR mapping strategies, it does not really attack the problem that I am addressing, namely the automated and exhaustive synthesis of the equivalence classes of mixed OR mapping specifications.

\end{comment}

\section{Summary}
\label{conclusion}

While a wealth of research has been performed on bridging application models and databases to address the {\em impedance mismatch} problem, little has been done on automated support for the derivation of mapping specifications for ORM frameworks.
This chapter presents a novel approach that substantially supports automatic generation of such mapping specifications to deliver the quality of expert-hand-crafted mappings and the productivity benefits of fully automated techniques.
This approach ultimately promises to reduce the engineering personnel costs involved in producing high-quality modern software systems.
The new mapping approach exposes many interesting research challenges.
These challenges include exploring symmetry breaking techniques customized for the specific domain of OR mappings to reduce the size of the solution space
and integrating the mapping compiler with industrial object-relational mapping tools.


==> copyright.tex <==
\ifwww
\chapter*{Copyright} 
\else
\newpage
\thispagestyle{empty}
\vspace*{\fill}
\fi

\begin{center}
\copyright\ Copyright 
\Month \Year \\
John Q.\ Public\\
All rights reserved\\
\end{center}

\ifwww\else
\vspace*{\fill}
\fi


==> glossary.tex <==
\chapter{Glossary}
\label{chap:glossary}

Definitions are collected here for easy reference.  In general, the
accepted definitions for terms are used, although some terms are used
in a more restricted sense than their usual interpretation.

\begin{description}

\item[xxxxxxxx xxxxxxxxxxx] x xxxxx xxxx xxx xxxxxxxxxxxx xxxx xxx 
xxxxxx xxxxx xxxxxxxx xxxxx xx xxxxxxxxxx xxx xxxxxxxxxx xx xxx xxxxx
xx xxxxxxx xxxx xxxx xxxxxxx.  xxxxxxxxxx xxx xx xx x xxxx xxxx xxxxx,
xxx xxxxxxx, xx xx xxxxxxxxxxx xxx xxxx xxx xx xxxxxxxxx xxxxxxxxxx,
xx xx x xxxxx xxxx xxxxx xx xx xxxxxxxxxxx xxxxx xxxx xx xxxxxxxx xx x
xxxxxxxxx xxxxxxxx xx x xxxxxxxx (xxx xxxxxxx, x xxxxx xxxxxx
xxxxxxxxxxx xxx xxxx xxxxxx xx ``xxxxx xx'' xxxxx xxxxx xxxxxxx).

\item[xxxxxxxxx xxxxxxx] x xxxxx-xxxx xxxxx-xxxxx xxx xxxxx xxxx xxxxxx 
xxxxxx xx xxxxx xxxxxxxx xxx x xxxxxxxxx xxx xxxxxxxx xx xxx xxxxxxxxx
xxxxx xxxxxxxxxxx xxxxx xxxxxx xxxx xxxxxxxxx.

\item[xxxxxxxxxxx] x xxxx-xxxxx xxxxxxx xxxxxxxx xx xxxxx x xxxxxxxx 
xxxxxxx.  xxxxxxxx xxxxxxxxxxxx xxx xx xxxxxxxxxxx xx xxxxxxxx
xxxxxxxxx, xx xxxx xxxxxxxxxxxx xx xxx xx xxxxxxx xxxx xx xxxxxxxxxxx
xx xxxxxxxxxxx xx x xxxxxx xxxxxxx.

\item[xxxx xxxxxx] x xxxxxxxx xxxxxxxxxx xxxxxx xx xxxxx xx 
xxxxxxx xxx xxxxxxxxxx xx xxxxxxxx.  xxxxxxxxxxxx, xx xxxxx xx xxxxxxx
xx xxxxxxxxxx.

\item[xxxxxx-xxxx xxxxxxxx] xxx-xxxxx xxxxxxxxx xxxxxx xxxxxxxx
xxxx xxx xxxxxx xxxxxxxx xxxx, xxx xx xxxxxxxxx xx, xxx xxxxxx
xxxxxxxxx xx x xxxxxxx-xxxxxxx xxxxxxxxx xxxxxx.

\item[xxxxxx xxxxxx] xxxxxxxxx x xxx xx xxxxx xx xxxxxxxxx xxxxxx 
xxxxxxxxxxxxx xx xxxxxxxxx xx xxx xxx xx xxxxxxxxxxxx xxxx xxxx xx
xxx, xxx xxxxx xxxxxxxx xxxxxxxxxxx.  xxxx xxxxxxx x xxxxxx
xxxxxxxxxxxxxx xxxxxxxx.

\item[xxxxxxxx] x xxxx, xxxxxxx xxxxxxxxxx xxxxxxx, xx xxxxx x xxxx-xxxx
xxxxxxxxxxx xxxx xxxxxxxx.

\end{description}

